Cumulative Message Authentication Codes for Resource-Constrained IoT Networks

In resource-constrained IoT networks, the use of conventional message authentication codes (MACs) to provide message authentication and integrity is not possible due to the large size of the MAC output. A straightforward yet naive solution to this problem is to employ a truncated MAC which undesirably sacrifices cryptographic strength in exchange for reduced communication overhead. In this paper, we address this problem by proposing a novel approach for message authentication called \textit{Cumulative Message Authentication Code} (CuMAC), which consists of two distinctive procedures: \textit{aggregation} and \textit{accumulation}. In aggregation, a sender generates compact authentication tags from segments of multiple MACs by using a systematic encoding procedure. In accumulation, a receiver accumulates the cryptographic strength of the underlying MAC by collecting and verifying the authentication tags. Embodied with these two procedures, CuMAC enables the receiver to achieve an advantageous trade-off between the cryptographic strength and the latency in processing of the authentication tags. Furthermore, for some latency-sensitive messages where this trade-off may be unacceptable, we propose a variant of CuMAC that we refer to as \textit{CuMAC with Speculation} (CuMAC/S). In addition to the aggregation and accumulation procedures, CuMAC/S enables the sender and receiver to employ a speculation procedure for predicting future message values and pre-computing the corresponding MAC segments. For the messages which can be reliably speculated, CuMAC/S significantly reduces the MAC verification latency without compromising the cryptographic strength. We have carried out comprehensive evaluation of CuMAC and CuMAC/S through simulation and a prototype implementation on a real car.

==> sec5_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We firstly highlight the advantages of CuMAC by comparing it with the prior art. We then evaluate the performance of CuMAC in an energy-constrained network application and a bandwidth-constrained network application. These two applications have very different constraints, but they share a common requirement---i.e., messages need to be protected using short tags---that illustrates the utility of CuMAC. 

\subsection{Comparison with the Prior Art}


\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=2\linewidth]{Figures/accumulated_security_vs_delay.eps}
    \caption{Trade-off between cryptographic strength and delay.}
    \label{fig:accumulating-security_vs_delay}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=2\linewidth]{Figures/packetDrop_vs_authentication.eps}
    \caption{Effect of unreliable communication channel.}
    \label{fig:packetDrop_vs_authentication}
\end{subfigure}
\caption{Comparison of CuMAC with the prior art.}
\end{figure}

We evaluate the performance of CuMAC by comparing it with three other schemes from the prior art: the truncated MAC \cite{Szi08}, the compound MAC \cite{Nil08}, and the aggregate MAC \cite{Kat08}. For all four schemes, AES-CMAC with a MAC output of 128 bits is utilized as the underlying MAC algorithm. We set the size of the tag in all the four schemes to 16 bits. In the truncated MAC scheme, each MAC is truncated to 16 bits, and transmitted as the tag. In the compound MAC scheme, a compound MAC of 128 bits is computed over eight messages. In the aggregate MAC scheme, an aggregate MAC of 128 bits is computed by aggregating the MACs of eight messages. The compound MAC and the aggregate MAC are divided into eight segments each of size 16 bits, and transmitted in each of the eight packets as the tag. In CuMAC, each MAC of 128 bits is divided into eight segments each of size 16 bits, and each tag is generated by aggregating segments of seven previously transmitted messages and the current message. 

Figure~\ref{fig:accumulating-security_vs_delay} presents the cryptographic strengths of four schemes versus their authentication delay. In the figure, we observe that CuMAC provides real-time authentication with cryptographic strength of 16 bits, which is the same for truncated MAC. As more packets are received, partially accumulated authentication is achieved and CuMAC provides gradually increased cryptographic strength.  Finally, CuMAC provides full authentication with cryptographic strength of 128 bits, which is the same as compound/aggregate MAC.

Most importantly, findings shown in Figure~\ref{fig:accumulating-security_vs_delay} highlight one critical advantageous attribute of CuMAC. CuMAC enables a receiver to make a trade-off between (accumulated) cryptographic strength and authentication delay. In some latency-tolerant applications, this attribute provides the receiver with operational flexibility to vary the security level and/or packet processing delay based on particular needs of a protocol or rules prescribed by network traffic processing policies. 

Further, we evaluate the effect of unreliable communication channel on the four schemes in Figure~\ref{fig:packetDrop_vs_authentication}. The unreliability of the channel is measured by the packet drop rate which is equal to the ratio of the lost packets and the total number of transmitted packets. The performance of each scheme is measured in terms of the packet processing rate which is equal to the ratio of successfully authenticated packets at the receiver and the total number of transmitted packets. We note that although the packet processing rates in CuMAC and the truncated MAC are equal (Figure~\ref{fig:packetDrop_vs_authentication}), the cryptographic strengths for their full authentication are 128 bits and 16 bits, respectively (Figure~\ref{fig:accumulating-security_vs_delay}).

Further, in Figure~\ref{fig:packetDrop_vs_authentication}, we observe that the compound/aggregate MAC can enable processing of significantly lower number of packets than CuMAC. This is because in compound/aggregate MAC, the verification of a MAC requires the receiver to receive \emph{all} of the packets that contain the messages utilized to compute that particular MAC, and loss of any one of those packets leads to the failure in processing of other packets. This implies that given the packet drop rate of $\rho$, the packet processing rate can be represented by $(1-\rho)$ in CuMAC, but $(1-\rho)^{n}$ in the compound/aggregate MAC. Hence, for a typical packet drop rate $\rho = 10\%$ and $n=8$, the packet processing rate in the compound/aggregate MAC is around $43\%$ which is an unacceptable rate in a typical network.


\subsection{Advantages in an Energy-Constrained Network}
\label{sec:evaluation:energy}

We consider an air quality monitoring system which consists of a base station and multiple sensors nodes distributed over a large area \cite{Sig17}. Each sensor node utilizes the Sigfox protocol to send the air quality data to the base station once in every hour \cite{Roh15}. The data is examined at the base station and finally made available to the responsible authorities. In this application scenario, there are two important performance requirements---(1) \textit{service life}: each battery-operated sensor node needs to operate for a few years independently without any physical access which means that the network is energy-constrained; and (2) \textit{robust authentication}: message authentication scheme is needed to ensure verification of received data despite losing some packets. Note that in this scenario, the latency requirement is not stringent as the data is collected and analyzed at the base station with some inherent delay.

\subsubsection{Service Life} 
We evaluate the effect of appending an authentication tag in each packet on the service life of a sensor node, which is equal to its battery life. To compute the service life, we utilize the charge consumption data from a Sigfox compliant transceiver IC produced by ON Semiconductor \cite{On18}. Table~\ref{tab:Sigfox} presents the parameters utilized in the computation of the service life. We employ two 1.5 V Alkaline C batteries connected in series. Each battery holds a charge of 8000 mAh. The transmission time in every hour is limited to 2 seconds, and hence the device is considered to be in sleep almost all the time. We ignore the battery self discharge in this calculation. 

\begin{table}[t]
\centering
\caption{Parameters utilized for computing the service life of a sensor node in a Sigfox network.}
\label{tab:Sigfox}
\renewcommand{\arraystretch}{1.2}
\scalebox{0.9}{
\begin{tabular}{|l|c|}
\hline
Battery capacity                 					& 8000 mAh $\times$ 3600 s/h   = 28800 C                		\\ \hline
Sleep charge                     					& 1.3 $\mu$A $\times$ 86400 s/day  = 0.11 C/day 				\\ \hline
Packet transmission rate                           	& 1 packet/h = 24 packets/day 									\\ \hline
Packet transmission without payload					& 0.20 C 														\\ \hline
Payload transmission								& 0.002 C/bit 													\\ \hline
\end{tabular}}
\end{table}

Figure~\ref{fig:Life_vs_MacLen} presents the service life of a sensor node for different sizes of message and authentication tag. We observe that by appending authentication tags in transmitted packets, each sensor node consumes a significantly more energy on data transmission which shortens the service life. Specifically, we consider a 48-bit message without tag as the benchmark which results in the service life of around 11 years. Figure~\ref{fig:Life_vs_MacLen} illustrates that in comparison to this benchmark, utilizing the conventional MAC of size 128 bits results in a significant loss of around 45\% of service life. However, CuMAC can utilize the 16-bit tag in each packet without compromising the cryptographic strength (128 bits) for full authentication, and with a modest (around 10\%) reduction in the service life as compared to the benchmark. Hence, for the LPWAN (like Sigfox) where the size of the tag in each packet is usually limited due to the energy constraints, we assert that CuMAC is a much more viable solution for message authentication than the full-size conventional MAC.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figures/Life_vs_MacLen.eps}
\caption{Effect of size of message and authentication tag on the service life of a sensor node in a Sigfox network.}
\label{fig:Life_vs_MacLen}
\end{figure}

\subsubsection{Robust Authentication}

Recall that in Sigfox, the sender becomes aware of the lost packet when it does not receive the acknowledgement from the receiver. Since Sigfox does not support retransmission of packets, the authentication scheme needs to be robust against packet drops. In CuMAC, the packet counter readily handles such cases, and ensures synchronization of packets between the sender and receiver. This implies that with CuMAC, all received messages can be authenticated with the cryptographic strength of 128 bits, albeit with some delay. However, in this application, the truncated MAC cannot provide high cryptographic strength as shown in Figure~\ref{fig:accumulating-security_vs_delay}, and the compound/aggregate MAC cannot provide robust authentication to all received packets as shown in Figure~\ref{fig:packetDrop_vs_authentication}. 


\subsection{Advantages in a Bandwidth-Constrained Network}

\begin{table}[t]
\centering
\caption{Distribution of size and period of messages in CAN.}
\label{tab:dist_msg}
\renewcommand{\arraystretch}{1.2}
\begin{minipage}[t]{\linewidth}
\centering
\scalebox{0.85}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Size}	& $1$ byte 	& $2$ bytes 	& $4$ bytes 	& $6$ bytes   \\ \hline
\textbf{Share}  & $35~\%$ 	& $49~\%$ 	& $13~\%$ 	& $3~\%$      \\ \hline
\end{tabular}}
\end{minipage}

\vspace{10pt}

\begin{minipage}[t]{\linewidth}
\centering
\scalebox{0.85}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Period} & $5$ ms  & $10$ ms & $20$ ms & $50$ ms & $100$ ms & $200$ ms & $1000$ ms	\\ \hline
\textbf{Share}	& $7~\%$ 	& $25~\%$	& $25~\%$	& $3~\%$	& $20~\%$	 & $1~\%$	  & $19~\%$ 	\\ \hline
\end{tabular}
}
\end{minipage}
\end{table}

We consider the CAN bus as an illustrative bandwidth-constrained network. We simulate the performance of the CAN bus when the authentication tag along with the message is inserted in the CAN packets. Table~\ref{tab:dist_msg} illustrates the distribution of the size and the period of messages utilized in the simulation. This distribution is based on the open-source benchmark presented by Kramer et al. \cite{Kra15}. The bus speed utilized in the simulation is $500$~kbps. In the simulation, we let the maximum size of the message to be 6 bytes which means 2 bytes (16 bits) of tag can be readily inserted in the data field. An 18-bit packet counter is inserted in the CAN identifier field \cite{Szi08,Ued15}. To communicate the full 128-bit tag, an ECU may employ the \textit{trailing MAC} scheme in which the ECU needs to transmit two extra packets with the tag for each packet with the message~\cite{Gro12}. Recall that a maximum of 64 bits of tag can be transmitted in one CAN packet. In the above scenario, we evaluate two performance metrics of the CAN bus: \textit{bus load} and \textit{message processing delay}.

\subsubsection{Bus Load}
The bus load is a critical parameter for evaluating the overall latency performance of the CAN bus. Typically, the CAN bus load is between $30~\%$ to $40~\%$, but with systematic approaches based on scheduling analysis, the bus load can be increased to around $80~\%$ \cite{Dav07}. The bus load is directly proportional to the number of supported messages on the CAN bus. A high bus load may increase the latency of messages that may lead to problems, such as car functions being delayed and high possibility of communication fault situations \cite{Zag18}. Hence, it is critical to keep the bus load low.

\begin{figure}[t]
\includegraphics[width=\linewidth]{Figures/BusUtil_vs_MsgNum.eps}
\caption{Effect of size of message and authentication tag on the CAN bus load.}
\label{fig:bus_util}
\end{figure}


Figure \ref{fig:bus_util} illustrates the effect of increasing the number of messages and inserting authentication tags in the CAN packet on the CAN bus load. We observe that at a typical bus load of $40~\%$, the number of supported messages without authentication is $60$. While maintaining the same bus load, CuMAC with a $16$-bit tag is able to support $45$ messages, but a trailing MAC with a $128$-bit tag supports only $12$ messages. Further, considering the maximum bus load of $80~\%$, the maximum number of messages supported by the bus with a $16$-bit tag is $91$, but that with a $128$-bit tag is only $27$. This means that to support $91$ messages, a vehicle needs only one CAN bus when the messages are authenticated using CuMAC, but it needs three CAN buses when the messages are authenticated using a full-size MAC. Note that increasing the number of CAN buses increases the overall cost of the vehicle.

\subsubsection{Message Processing Delay}
Message processing delay is an important design metric for the CAN bus which supports safety-critical functions of a vehicle \cite{Dav07}. The major components of this delay includes the delay in the generation of the authentication tag at the sender, communication of the CAN packet over the bus, and then verification of the authentication tag at the receiver. We note that although the CAN bus enforces strict message processing deadlines, the individual communication delay encountered by each \textit{message type} (which denotes all messages with the same message identifier) on the bus can vary significantly between 5 ms and 1000 ms~\cite{Zag18}. Also, recall that CuMAC supports accumulation of cryptographic strength as per the flexible delay requirement as shown in Figure~\ref{fig:accumulating-security_vs_delay}. This implies that with CuMAC, some message types can be authenticated with high cryptographic strength. Unlike CuMAC, the truncated MAC does not support accumulation of cryptographic strength, and the compound/aggregate MAC cannot provide real-time authentication guarantee which is essential for the CAN bus. 

==> sec6_implementation.tex <==
\section{Implementation Results}
\label{sec:implementation}

We discuss the results from the experiments performed with a prototype implementation. These results are also utilized to compare CuMAC with the MAC schemes in the prior art. 

\input{Tables/implementation_table.tex}


\subsection{Details of the Prototype Implementation}

\begin{figure}[t]
\centering
\includegraphics[width=0.75\linewidth, angle=0]{Figures/testbed.eps}
\caption{Prototype connected to a car's CAN bus.}
\label{fig:testbed}
\end{figure}

Figure~\ref{fig:testbed} illustrates the prototype implementation and the setup that were used for running our experiments. The prototype implementation comprised of two ECU prototypes connected to the on-board diagnostics (OBD) port of the CAN bus (with the bus speed of $500$~kbps) of a 2016 Toyota Corolla LE. The ECU prototype consisted of an Arduino UNO board and a Seeed studio CAN shield. The Arduino UNO board was used to emulate the controller unit of an ECU, and the Seeed studio CAN shield worked as the interface between the Arduino UNO board and the CAN bus. The Arduino UNO board utilizes an Atmel ATmega328P chip, which includes a low-power 8-bit micro-controller running at 16~MHz clock speed along with a 32~KB flash memory and a 2~KB RAM. These specifications of the ECU prototype are representative of a typical state-of-the-art automotive-grade controller \cite{Mur16}.

With the above experimental setup, we compared five schemes: the trailing MAC, the truncated MAC, the compound MAC, the aggregate MAC and CuMAC. For all five schemes, AES-CMAC with a MAC output of 128 bits was utilized as the underlying MAC algorithm. We utilized an open-source cryptography library~\cite{github_aes} to implement AES-CMAC. We found that the computation time (calculated by averaging the computation time over 1000 executions) of generating a MAC was 0.786 ms. For the truncated MAC, the compound MAC, the aggregate MAC and CuMAC, the size of the tag was set to 16 bits, and the message and tag were inserted into the data field of the same CAN packet. For the trailing MAC, the 128-bit MAC was split into two tags of 64 bits, and inserted into the data fields of two consecutive CAN packets. These packets were transmitted immediately after the CAN packet containing only the message. 

To evaluate the delay performance, we utilized one ECU prototype (called Tx-ECU) to transmit 6-byte messages with the tags on the CAN bus, and another ECU prototype (called Rx-ECU) to measure the end-to-end delay. In the experiment, the Rx-ECU requested the Tx-ECU (through an external synchronization channel) to send a message, and started the timer. The Rx-ECU stopped the timer after verifying the tag and authenticating the message. The delay was measured as the time between starting the timer and stopping the timer. Also, we let the message processing deadline for the message type utilized in the experiment be 50~ms. Note that the processing deadline represents the time within which the authentication tags corresponding to the message are expected to be generated, communicated and verified.



\subsection{Results}


Table~\ref{tab:prototype} summarizes the results from the experiments. The end-to-end delay shown in the table is the worst case delay in processing 1000 CAN messages. The table also presents the cryptographic strengths for real-time, full and partially accumulated authentication in each scheme. From Table~\ref{tab:prototype}, we observe that: (1) In comparison to the truncated MAC, additional 112 bytes of storage is required to store the segments of the MACs of seven previous messages in CuMAC; (2) Unlike the trailing MAC, CuMAC does not increase the bus load significantly; (3) Unlike the compound MAC and the aggregate MAC, CuMAC provides real-time authentication; and (4) In comparison with the truncated MAC, the compound MAC and the aggregate MAC schemes, CuMAC provides higher cryptographic strength for partially accumulated authentication within the processing deadline.

==> sec7_security_proof.tex <==
\section{Security Analysis}
\label{sec:security}

In this section we present formal security definition and proof for CuMAC. 

\subsection{Security Definition}

The security definition for CuMAC is based on the notion of unforgeability under chosen message attack (uf-cma). We present the following uf-cma-$r$ experiment, where the parameter $r$ indicates the number of segments accumulated for tag verification. 

\vspace{5pt}
\noindent $\mathbf{Exp}_{\mathsf{CuMAC}}^{\textnormal{uf-cma-}r}(\adv,\lambda,q)$

\begin{itemize}
\item[] $\mathtt{k}\gets \mathsf{KeyGen}(1^\lambda)$


\item[] Invoke an adversary $\adv$ who can make up to $q$ queries to the tag generating oracle of CuMAC, $O_{\mathsf{CuMAC}}(\mathtt{k},\cdot)$. 

\item[] $\adv$ queries $O_{\mathsf{CuMAC}}(\mathtt{k},\cdot)$ with $n$ arbitrarily chosen messages and receives their corresponding tags in response.

\item[] $\adv$ outputs a set of $n$ pairs $\left(\set{m_i}_{i=1}^{n},\set{\tau_i}_{i=1}^{n}\right)$.

\item[] Return 1 if $\mathtt{valid} \gets \mathsf{TagVerify}\left(\mathtt{k},i,m_i,\tau_i \right)$ for all $1\leq i \leq n$, and $\adv$ did not make the query for $m_{i^*}$ to $O_{\mathsf{CuMAC}}(\mathtt{k},\cdot)$, where $i^* = n-r+1$.

\item[] Return 0 otherwise.
\end{itemize}
\vspace{5pt}

Using the above experiment, we present the following security definition where the probability is denoted by $\prob{}$.

\begin{definition}
\label{def:CuMAC_security}
CuMAC is $(t,q,\epsilon,r)$-uf-cma secure if for any probabilistic polynomial time (PPT) adversary $\adv$ running in time $t$, $\prob{\mathbf{Exp}_{\mathsf{CuMAC}}^{\textnormal{uf-cma-}r}(\adv,\lambda,q)=1}\leq \epsilon$.
\end{definition}

We utilize the above uf-cma-$r$ security model to define the cryptographic strengths for full, partially accumulated and real-time authentication. If CuMAC is $(t,q,\epsilon, n)$ secure, i.e., $r=n$, then CuMAC is secure in terms of full authentication. Similarly, if CuMAC is $(t,q,\epsilon, r)$ secure for all $1 < r < n$, then the scheme is secure for partially accumulated authentication; and if CuMAC is $(t,q,\epsilon, 1)$ secure, i.e., $r=1$, then the scheme is secure in terms of real-time authentication.

\subsection{Security Proof}

Here, we present the security proof for CuMAC which closely follows the proof for the aggregate MAC scheme \cite{Kat08}. Let CuMAC be instantiated with parameters $(l,n)$, i.e., each MAC is divided into $n$ segments, each of length $l$ bits.

\begin{theorem}\label{theorem:CuMAC}
For any $t,q \in \NN$ and $\epsilon > 0$, if the underlying deterministic MAC generation algorithm, $\mathsf{MacGen}$, is $(t,q,\epsilon)$-uf-cma secure, then CuMAC with parameters $(l,n)$ is $(t',q',\epsilon',r)$-uf-cma secure, where 
\begin{align*}
t' \approx t, ~~~~ q' = \frac{q-n+1}{n}, ~~~~\text{and}~~~~ \epsilon' = 2^{l(n-r)} \cdot \epsilon.
\end{align*}
\end{theorem}

\begin{IEEEproof}
Let there be an adversary $\adv$ which succeeds to create a forgery of an authentication tag for CuMAC with a non-negligible probability. We construct a simulator $\sdv$ that interacts with the adversary $\adv$ and creates a forgery of a MAC for the $\mathsf{MacGen}$ algorithm with a non-negligible probability. 

Let CuMAC and the $\mathsf{MacGen}$ algorithm utilize the same secret key $\mathtt{k}$ which is unknown to the adversary $\adv$. Also, let the underlying MAC of a message in CuMAC be retrieved by a query to the MAC generating oracle $O_{\mathsf{MacGen}}(\mathtt{k},\cdot)$. In this way, $\sdv$ perfectly simulates the tag generating oracle $O_{\mathsf{CuMAC}}(\mathtt{k},\cdot)$, and hence the uf-cma-$r$ experiment for CuMAC. Suppose the uf-cma-$r$ experiment for CuMAC returns $1$ with the probability $\epsilon'$ in time $t'$, where an adversary $\adv$ outputs a successful forgery $\left(\set{m_i}_{i=1}^{n}, \set{\tau_i}_{i=1}^{n} \right)$ after $q'$ queries to $O_{\mathsf{CuMAC}}(\mathtt{k},\cdot)$ simulated by $\sdv$. 

To create a forgery of a MAC for the $\mathsf{MacGen}$ algorithm, the simulator $\mathcal{S}$ proceeds as follows. Given $i^* = n-r+1$, the simulator $\mathcal{S}$ queries $O_{\mathsf{MacGen}}(\mathtt{k},\cdot)$ for the MAC of $m_i$, and obtains the corresponding $\sigma_i$ for all $i \in [1,n]$ and $i \neq i^*$. It divides each MAC into $n$ segments as shown in equation~\eqref{eq:segment}. Then, for each $k\in [1,r]$, it recovers the MAC segment of the message $m_{i^*}$ by removing the mask by the MAC segments of other messages as follows.
\begin{align} \label{eq:sec_rec_p}
s_{i^*}^k \gets \tau_{i^*+k-1} \oplus \bigoplus_{j=1,j\neq k}^{n}  s_{i^*-j+k}^j.
\end{align}
By following the above procedure, the simulator $\mathcal{S}$ recovers $r$ MAC segments. Since $i^* = n-r+1$, the simulator $\mathcal{S}$ cannot recover the segments $s_{i^*}^k$ with $k \geq r+1$. Hence, it makes a random guess for the rest of the $n-r$ segments, such that $\widetilde{s}_{i^*}^k \sample \set{0,1}^{l}$ for all $k \in [r+1,n]$. Finally, the simulator $\mathcal{S}$ creates a fresh forgery for the $\mathsf{MacGen}$ algorithm, by concatenating all recovered and guessed segments. The probability that such forgery is correct is $2^{-l(n-r)}$.

To achieve the forgery of $\mathsf{MacGen}$ as shown above, the simulator $\mathcal{S}$ conducts at most $n \cdot q'$ queries to $O_{\mathsf{MacGen}}(\mathtt{k},\cdot)$ to answer $q'$ queries by $\adv$ to $O_{\mathsf{CuMAC}}(\mathtt{k},\cdot)$. In order to compute operations in equations~\eqref{eq:sec_rec_p}, the simulator $\mathcal{S}$ conducts at most $n-1$ queries to $O_{\mathsf{MacGen}}(\mathtt{k},\cdot)$ to obtain $\set{\tau_i}_{i=1,i\neq i^*}^{n}$. Therefore, if for an adversary $\adv$ running in time $t'$ can have $\prob{\mathbf{Exp}_{\mathsf{CuMAC}}^{\textnormal{uf-cma-}r}(\adv,\lambda,q')=1}\leq \epsilon'$, then $\sdv$ can leverage $\adv$ to break the $\mathsf{MacGen}$ algorithm, in time $t'$ plus the time required to evaluate equation~\eqref{eq:sec_rec_p}, by making $n \cdot q'+n-1$ queries, and with probability $2^{-l(n-r)} \cdot \epsilon'$. Hence, if the $\mathsf{MacGen}$ algorithm, is $(t,q,\epsilon)$-uf-cma secure, then CuMAC is $(t',q',\epsilon',r)$-uf-cma secure, where $t' \approx t$, $q' = \frac{q-n+1}{n}$, and $\epsilon' = 2^{l(n-r) \cdot \epsilon}$.
\end{IEEEproof}
